DEPT: Decoupled Embeddings for Pre-training Language Models

Language Model pre-training uses broad data mixtures to enhance performance across domains and languages. However, training on such heterogeneous text corpora requires extensive and expensive efforts. Since these data sources vary significantly in lexical, syntactic, and semantic aspects, they cause negative interference or the ``curse of multilinguality''. To address these challenges we propose a communication-efficient pre-training framework, DEPT. Our method decouples embeddings from the transformer body while simultaneously training the latter on multiple data sources without requiring a shared vocabulary. DEPT can: (1) train robustly and effectively under significant data heterogeneity, (2) minimize token embedding parameters to only what the data source vocabulary requires, while cutting communication costs in direct proportion to both the communication frequency and the reduction in parameters, (3) enhance transformer body plasticity and generalization, improving both average perplexity (up to 20%) and downstream task performance, and (4) enable training with custom optimized vocabularies per data source. We demonstrate DEPT's potential via the first vocabulary-agnostic federated pre-training of billion-scale models, reducing communication costs by orders of magnitude and embedding memory by 4-5x.

==> algorithms/mclr_full.tex <==




\begin{algorithm}
\caption{Meta-Learning Optimization with Embedding Subsampling and Specialization}
\begin{onehalfspace}
\begin{algorithmic}[1]
\Require{$S$: set of $K$ data sources, $T$: number of meta-update rounds}
\Require{$\theta_0$: initial transformer blocks, $\phi_0$: optional initial token embedding matrix}
\Require{$\{\mathcal{D}_k\}_{k=1}^K$: source-specific datasets, $\{\mathcal{V}_k\}_{k=1}^K$: source-specific vocabularies}
\Require{\texttt{InnerOPT}: inner loop optimization algorithm, \texttt{OuterOPT}: outer loop algorithm}
\Ensure{Meta-learned model $\theta_T$, optional global token embedding matrix $\phi_T$}

\For{each meta-update round $t = 1, 2, \ldots, T$}
    \State{Randomly select a subset $S_t\subseteq S$ of data sources for round $t$}
    \For{each data source $k \in S_t$ \textbf{in parallel}}

        % \State{\colorbox{red!30}{$\phi_t^k \gets \phi_{t-1}[V_k]$}} \Comment{Trim global token embeddings}
        % \State{\colorbox{blue!30}{$\phi_t^k \gets \phi_{t-1}$}}  \Comment{Get latest global token embeddings}
        
        % \If{\textcolor{teal}{Subsampling}}
        % \ElsIf{\textcolor{cyan}{Specialization}}
        %     \State{\textcolor{cyan}{$\phi_t^k \gets \Call{RandomInit}{V_k}$}}  \Comment{Initialize new specialized token embeddings}
        %     \If{\textcolor{cyan}{specialized embedding matrix $\phi_k$ exists}}
        %         \State{\textcolor{cyan}{$\phi_t^k \gets \phi_k$}}  \Comment{Use existing specialized token embeddings}
        %     \EndIf
        % \EndIf
        
        \State{\colorbox{red!30}{$\theta_t^k, \phi_t\vert_{\mathcal{V}_k} \gets \texttt{InnerOPT}(\theta_{t-1}, \phi^k_{t-1}, \mathcal{D}_k),~\phi_{t-1}\vert_{\mathcal{V}_k} = \texttt{Trim}(\phi_{t-1},V_k)$}}
        \State{\colorbox{blue!30}{$\theta_t^k, \phi_t^k \gets \texttt{InnerOPT}(\theta_{t-1}, \phi_{t-1}, \mathcal{D}_k)$}}
        \State{$\Delta \theta_t^k \gets \theta_t^k - \theta_{t-1}$}  \Comment{Compute parameter update}
        \State{\colorbox{red!30}{$\Delta \phi_t\vert_{\mathcal{V}_k} \gets \phi_t\vert_{\mathcal{V}_k} - \phi_{t-1}\vert_{\mathcal{V}_k}$}}  \Comment{Compute token embedding update}
        \State{\colorbox{blue!30}{$\Delta \phi_t^k \gets \phi_t^k - \phi_{t-1}$}}  \Comment{Compute token embedding update}
        % \If{\textcolor{teal}{Subsampling}}
        % \State{\textcolor{teal}{$\Delta \phi_t^k \gets \phi_t^k - \phi_{t-1}[\mathcal{V}_k]$}  \Comment{Compute token embedding update}}
        % \EndIf

    \EndFor
    \State{$\theta_t \gets \texttt{OuterOPT}(\theta_{t-1}, \{\Delta \theta_t^k\}_{k \in S_t})$}
    \State{\colorbox{red!30}{$\phi_t \gets \texttt{OuterOPT}(\phi_{t-1}, \{\Delta \phi_t\vert_{\mathcal{V}_k}\}_{k \in S_t})$}}
    \State{\colorbox{blue!30}{$\phi_t \gets \texttt{OuterOPT}(\phi_{t-1}, \{\Delta \phi_t^k\}_{k \in S_t})$}}
    % \If{\textcolor{teal}{Subsampling}}{
    % \State{\textcolor{teal}{$\phi_t \gets \phi_{t-1}$} } \Comment{Initialize with previous token embeddings}
    % \For{\textcolor{teal}{each data source $k \in S_t$}}
    %     \State{\textcolor{teal}{$\phi_t[\mathcal{V}_k] \gets \texttt{OuterOPT}(\phi_{t-1}[\mathcal{V}_k], \Delta \phi_t^k)$}}
    % \EndFor
    % }
    % \EndIf
\EndFor
\State{\Return{$\theta_T, \phi_T$}}
\end{algorithmic}
\end{onehalfspace}
\end{algorithm}

==> tables/mc4_125M-pm.tex <==
\begin{table}[ht]
  \caption{ { \color{blue} Validation perplexity ($\downarrow$)  for our $12$-block models trained on \texttt{MC4} when using continued pre-training with proportional sampling starting from a pre-trained embedding matrix. When comparing against \cref{tab:mc4_125M_r}, we observe that \dept wins the losing comparisons when starting from random embeddings, indicating that this gap is driven by the embedding space being fitted to the high-resource languages despite the baselines having a \textbf{worse} transformer body.} } \label{tab:mc4_125M_pm} 
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
 & \multicolumn{9}{c}{\textbf{In-Distribution}} & \multicolumn{4}{c}{\textbf{Out-of-Distribution}} \\ \cmidrule(lr){2-10} \cmidrule(l){11-14} 
\textbf{\begin{tabular}[c]{@{}l@{}}Name\\ ({\scriptsize UNIGRAM-CE})\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ZH\\ ($9.8$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}UR\\ ($10.5$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MS\\ ($9.2$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}IT\\ ($7.7$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}SR\\ ($10.5$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LA\\ ($9$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}EN\\ ($7.5$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}SW\\ ($10$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg (In-D)\\ ($9.3$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}EL\\ ($14.4$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}HI\\ ($13.9$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DE\\ ($9.7$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg (OOD)\\ ($12.6$)\end{tabular}} \\ \cmidrule(lr){2-10} \cmidrule(l){11-14} 
\textbf{\texttt{UNIF}} & $62.9$ & $28.2$ & $54.1$ & $35.2$ & $43.8$ & $42.5$ & $52.4$ & $47.5$ & $45.8$ & $2317.4$ & $1797.7$ & $396.8$ & $1503.9$ \\
\textbf{\texttt{T} ($\boldsymbol{\tau = 0.3}$)} & $46.3$ & $37.4$ & $51.1$ & $\mathbf{22.7}$ & $55.5$ & $68.5$ & $35.3$ & $87.8$ & $50.6$ & $2576.3$ & $1706.9$ & $\mathbf{285}$ & $1522.7$ \\
\textbf{\texttt{PROP}} & $47.4$ & $\mathbf{25.7}$ & $45.9$ & $28$ & $\mathbf{39}$ & $\mathbf{39.5}$ & $42.6$ & $\mathbf{43.6}$ & $\mathbf{39}$ & $\mathbf{2038.2}$ & $1383.4$ & $323.1$ & $\mathbf{1248.2}$ \\ \cmidrule(lr){2-10} \cmidrule(l){11-14} 
\textbf{\glob} & $\mathbf{42.5}$ & $27.5$ & $\mathbf{36.5}$ & $28.6$ & $96.1$ & $84.6$ & $\mathbf{34.9}$ & $103.6$ & $56.8$ & $3680.1$ & $\mathbf{1173.9}$ & $343.4$ & $1732.4$ \\
\textbf{\trim} & $45$ & $30.7$ & $38.5$ & $29.8$ & $101.9$ & $87.6$ & $36.2$ & $106.7$ & $59.6$ & $3252.6$ & $1250.6$ & $355.8$ & $1619.7$ \\ \cmidrule(r){1-10} \cmidrule(l){11-14} 
\textbf{Min Imp (\%)} & $\mathbf{2.8}$ & $-19.5$ & $\mathbf{16}$ & $-31.1$ & $-161.2$ & $-121.6$ & $-2.4$ & $-144.9$ & $-52.8$ & $-80.6$ & $\mathbf{9.6}$ & $-24.8$ & $-38.8$ \\
\textbf{Max Imp (\%)} & $\mathbf{8.1}$ & $-7.2$ & $\mathbf{20.5}$ & $-25.6$ & $-146.1$ & $-114.1$ & $\mathbf{1.2}$ & $-137.8$ & $-45.7$ & $-59.6$ & $\mathbf{15.1}$ & $-20.5$ & $-29.8$ \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/mc4_125M-pr.tex <==
\begin{table}[ht]
\caption{ { \color{blue} Validation perplexity ($\downarrow$) for our $12$-block models trained on \texttt{MC4} when using continued pre-training with proportional sampling starting from randomly-initialized embeddings. \dept provides a better transformer body for \textbf{all} languages, outperforming baselines by up to $12.4\%$ on average for in-distribution data and $27.7\%$ for OOD data. }} \label{tab:mc4_125M_pr} 
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrrrrrrrrrrr@{}}
\toprule
 & \multicolumn{9}{c}{\textbf{In-Distribution}} & \multicolumn{4}{c}{\textbf{Out-of-Distribution}} \\ \cmidrule(lr){2-10} \cmidrule(l){11-14} 
\textbf{\begin{tabular}[c]{@{}l@{}}Name\\ ({\scriptsize UNIGRAM-CE})\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}ZH\\ ($9.8$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}UR\\ ($10.5$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}MS\\ ($9.2$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}IT\\ ($7.7$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}SR\\ ($10.5$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}LA\\ ($9$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}EN\\ ($7.5$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}SW\\ ($10$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}Avg (In-D)\\ ($9.3$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}EL\\ ($14.4$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}HI\\ ($13.9$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}DE\\ ($9.7$)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}Avg (OOD)\\ ($12.6$)\end{tabular}} \\ \cmidrule(r){1-10} \cmidrule(l){11-14} 
\textbf{\texttt{UNIF}} & $134.9$ & $88.1$ & $121.5$ & $49$ & $167.6$ & $191.6$ & $72.8$ & $792.1$ & $202.2$ & $11123.4$ & $7000.4$ & $1068.2$ & $6397.3$ \\
\textbf{\texttt{T} ($\boldsymbol{\tau = 0.3}$)} & $109$ & $78.1$ & $103.7$ & $43.6$ & $140.4$ & $146$ & $65.6$ & $690.4$ & $172.1$ & $9191.2$ & $5194.3$ & $833.4$ & $5073$ \\
\textbf{\texttt{PROP}} & $90.7$ & $72.6$ & $91.3$ & $38$ & $119$ & $131.8$ & $57.5$ & $472.5$ & $134.2$ & $9145.3$ & $5694.4$ & $740.1$ & $5193.3$ \\
\textbf{\act} & $107.7$ & $87$ & $102.1$ & $42.9$ & $135.8$ & $139.9$ & $64.7$ & $380.2$ & $132.5$ & $7412.8$ & $4667.8$ & $752.7$ & $4277.7$ \\ \cmidrule(r){1-10} \cmidrule(l){11-14} 
\textbf{\glob} & $\mathbf{72.2}$ & $\mathbf{58.3}$ & $\mathbf{77.3}$ & $\mathbf{32.3}$ & $\mathbf{97}$ & $\mathbf{110.8}$ & $\mathbf{49.3}$ & $353.9$ & $106.4$ & $6264.9$ & $\mathbf{2862.3}$ & $\mathbf{575.4}$ & $3234.2$ \\
\textbf{\trim} & $74.1$ & $59.2$ & $79$ & $33$ & $99.9$ & $113.1$ & $50.3$ & $\mathbf{333}$ & $\mathbf{105.2}$ & $6161.5$ & $3315$ & $598.4$ & $3358.3$ \\
\textbf{\spec} & $74.4$ & $59$ & $79.9$ & $33.6$ & $101.1$ & $112.7$ & $51.3$ & $348.6$ & $107.6$ & $\mathbf{5631.3}$ & $3064.1$ & $579.1$ & $\mathbf{3091.5}$ \\ \cmidrule(r){1-10} \cmidrule(l){11-14} 
\textbf{Min Imp (\%)} & $\mathbf{18}$ & $\mathbf{18.4}$ & $\mathbf{12.5}$ & $\mathbf{11.6}$ & $\mathbf{15.1}$ & $\mathbf{14.2}$ & $\mathbf{10.8}$ & $\mathbf{6.9}$ & $\mathbf{18.8}$ & $\mathbf{15.5}$ & $\mathbf{29}$ & $\mathbf{19.1}$ & $\mathbf{21.5}$ \\
\textbf{Max Imp (\%)} & $\mathbf{20.4}$ & $\mathbf{19.8}$ & $\mathbf{15.3}$ & $\mathbf{15}$ & $\mathbf{18.5}$ & $\mathbf{15.9}$ & $\mathbf{14.2}$ & $\mathbf{12.4}$ & $\mathbf{20.6}$ & $\mathbf{24}$ & $\mathbf{38.7}$ & $\mathbf{22.3}$ & $\mathbf{27.7}$ \\ \bottomrule
\end{tabular}%
}
\end{table}
